Einstein metrics on the full flag $F(n)$

Let $ M = G/K $ be a full flag manifold. In this work, we investigate the $ G$-stability of Einstein metrics on $M$ and analyze their stability types, including coindices, for several cases. We specifically focus on $F(n) = \mathrm{SU}(n)/T$, emphasizing $n = 5$, where we identify four new Einstein metrics in addition to known ones. Stability data, including coindex and Hessian spectrum, confirms that these metrics on $F(5)$ are pairwise non-homothetic, providing new insights into the finiteness conjecture.

==> secciones/G2.tex <==
In this section, we investigate the Einstein metrics on $G_2/T^2$, in this case $\dim \mathcal{M}_1^G=5$. In this particular scenario, all metrics are precisely documented in \cite[Theorem A]{ArvanitoChrysikosSakaneG2}, and we will present their $G$-stability.


The isotropy representation is given by
$$
\mg=\mg_1\oplus\mg_2\oplus\mg_3\oplus\mg_4\oplus\mg_5\oplus\mg_6,
$$
where $\mathfrak{m}_i$ corresponds to the $i$-th positive root, and furthermore, $\dim \mg_i=2$. Refer to \cite{ArvanitoChrysikosSakaneG2} for more details. In the same work, the authors demonstrated that the non-zero structural constants are given by
$$
[1\,2\,3]=[2\,4\,5]=[3\,4\,6]=[1\,5\,6]=\frac{1}{4} \quad \text{and}\quad [2\,3\,4]=\frac{1}{3}.
$$
\begin{theorem}\cite{ArvanitoChrysikosSakaneG2}
The full flag manifold $G_2/T^2$ admits exactly three $G_2$-invariant Einstein metrics (up to isometry). These metrics are specified as follows:
$$
\begin{aligned}
g_K&=(3,1,4,5,6,9),\\ g_1&\approx(1,0.2762,1.0347,1.0347,1,1.7895),\\
g_2&\approx(1,0.2173,1.0234,1.0234,1,0.7440),
\end{aligned}
$$ 
where the first one is Kähler, and the last two are given by approximate values.
\end{theorem}

Now we can compute the matrix $[L_{\mathfrak{p}}]$ to analyze their $G$-stability. We summarize the results in the following theorem.

\begin{theorem}
The metrics $g_K, g_1$ and $g_2$ are pairwise non-isometric, and their $G$-stability is presented in Table \ref{tab:metrics G2/T}.
\end{theorem}
\begin{proof}
To demonstrate that $g_K$ is non-homothetic to $g_1$ and $g_2$, observe that $\lambda_{\mathfrak{p}}(g_K)=0$, while $\lambda_{\mathfrak{p}}(g_1), \lambda_{\mathfrak{p}}(g_2)\neq 0$. Moreover, since $g_1$ and $g_2$ have different coindex, they are non-homothetic to each other.
\end{proof}

\begin{table}
    \centering
\begin{tabular}{| c | c | c | c | c | c | c | c |}
\hline
Name  & Propieties & $2\rho$ & $Sc_N$ & coindex & $\lambda_\pg$ &$\lambda_{\pg}^{max}$\\ \hline
$g_K$  & Non-deg. and unstable. & {\tiny$\tfrac{1}{6}$} & {\tiny $10497600^{\frac{1}{12}}\approx 3.8467$} & 2 & 0 & 1.028\\ \hline
$g_1$  & Non-deg. and unstable. & 0.7120 & 3.8423 & 3 & 0.2394 & 3.5930\\ \hline
$g_2$  & Non-deg. and unstable. & 0.8538 & 3.8106 & 2 & 0.1727 & 4.6410\\ \hline
\end{tabular}    
    \caption{$G$-stability of metrics on $G_2/T^2$.}
    \label{tab:metrics G2/T}
\end{table}
\begin{remark}
    Values with a decimal point are approximate values.
\end{remark}
